Estimation of Radio Channel Parameters in Case of an Unknown Transmitter

This paper investigates the estimation of radio channel parameters from receiver data, whereby the transmitter is fully unknown. We use a multipath model to describe the radio channel between transmitter and receiver. According to this model, we discuss the accessibility of parameters for estimation. Based on the Maximum-Likelihood principle, we derive a cost function. A second cost function is derived from the cross relation between the receiver channels. To estimate the parameters, we seek for the minimum of these cost functions. The performance of the presented cost functions are compared in simulations.

==> Figures/RMSE_AoA.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextA SNR in dB}%
\psfrag{014}[bc][bc]{\matlabtextA RMSE AoA}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $2$}%
\psfrag{002}[ct][ct]{\matlabtextB $4$}%
\psfrag{003}[ct][ct]{\matlabtextB $6$}%
\psfrag{004}[ct][ct]{\matlabtextB $8$}%
\psfrag{005}[ct][ct]{\matlabtextB $10$}%
\psfrag{006}[ct][ct]{\matlabtextB $12$}%
\psfrag{007}[ct][ct]{\matlabtextB $14$}%
\psfrag{008}[ct][ct]{\matlabtextB $16$}%
\psfrag{009}[ct][ct]{\matlabtextB $18$}%
\psfrag{010}[ct][ct]{\matlabtextB $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{012}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>

==> Figures/RMSE_Delay.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextA SNR in dB}%
\psfrag{014}[bc][bc]{\matlabtextA RMSE normalised delay}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $2$}%
\psfrag{002}[ct][ct]{\matlabtextB $4$}%
\psfrag{003}[ct][ct]{\matlabtextB $6$}%
\psfrag{004}[ct][ct]{\matlabtextB $8$}%
\psfrag{005}[ct][ct]{\matlabtextB $10$}%
\psfrag{006}[ct][ct]{\matlabtextB $12$}%
\psfrag{007}[ct][ct]{\matlabtextB $14$}%
\psfrag{008}[ct][ct]{\matlabtextB $16$}%
\psfrag{009}[ct][ct]{\matlabtextB $18$}%
\psfrag{010}[ct][ct]{\matlabtextB $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{012}[rc][rc]{\matlabtextB $10^{0}$}%
%
%% </ytick>

==> Figures/RMSE_EoA.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextA SNR in dB}%
\psfrag{014}[bc][bc]{\matlabtextA RMSE EoA}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $2$}%
\psfrag{002}[ct][ct]{\matlabtextB $4$}%
\psfrag{003}[ct][ct]{\matlabtextB $6$}%
\psfrag{004}[ct][ct]{\matlabtextB $8$}%
\psfrag{005}[ct][ct]{\matlabtextB $10$}%
\psfrag{006}[ct][ct]{\matlabtextB $12$}%
\psfrag{007}[ct][ct]{\matlabtextB $14$}%
\psfrag{008}[ct][ct]{\matlabtextB $16$}%
\psfrag{009}[ct][ct]{\matlabtextB $18$}%
\psfrag{010}[ct][ct]{\matlabtextB $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{012}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>

==> Figures/RMSE_Power.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextA SNR in dB}%
\psfrag{014}[bc][bc]{\matlabtextA RMSE normalised power}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $2$}%
\psfrag{002}[ct][ct]{\matlabtextB $4$}%
\psfrag{003}[ct][ct]{\matlabtextB $6$}%
\psfrag{004}[ct][ct]{\matlabtextB $8$}%
\psfrag{005}[ct][ct]{\matlabtextB $10$}%
\psfrag{006}[ct][ct]{\matlabtextB $12$}%
\psfrag{007}[ct][ct]{\matlabtextB $14$}%
\psfrag{008}[ct][ct]{\matlabtextB $16$}%
\psfrag{009}[ct][ct]{\matlabtextB $18$}%
\psfrag{010}[ct][ct]{\matlabtextB $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{012}[rc][rc]{\matlabtextB $10^{-1}$}%
%
%% </ytick>
